Understanding Domain Learning in Language Models Through Subpopulation Analysis

We investigate how different domains are encoded in modern neural network architectures. We analyze the relationship between natural language domains, model size, and the amount of training data used. The primary analysis tool we develop is based on subpopulation analysis with Singular Vector Canonical Correlation Analysis (SVCCA), which we apply to Transformer-based language models (LMs). We compare the latent representations of such a language model at its different layers from a pair of models: a model trained on multiple domains (an experimental model) and a model trained on a single domain (a control model). Through our method, we find that increasing the model capacity impacts how domain information is stored in upper and lower layers differently. In addition, we show that larger experimental models simultaneously embed domain-specific information as if they were conjoined control models. These findings are confirmed qualitatively, demonstrating the validity of our method.

==> background.tex <==
\section{Background}
\label{section:cca}
Our analysis is based on Canonical Correlation Analysis (CCA), which aims at projecting
two vector random variables into a joint space that maximizes their correlation.
More specifically, given two random variables $\rv{X}$ and $\rv{Z}$,
we find $\mat{U}$ and $\mat{V}$ such that for any $i \in [d']$ it holds that:
\begin{align}
\mathrm{Corr}(\mat{U}_i^{\top} \rv{X}, \mat{V}_i^{\top} \rv{Z})  = \max_{(\myvec{a},\myvec{b}) \in \mathcal{O}_i} \mathrm{Corr}(\myvec{a}^{\top} \rv{X}, \myvec{b}^{\top}\rv{Z}) ,\nonumber
\end{align}
\noindent where $\mathcal{O}_i$ is the set of pairs of vectors $(\myvec{a},\myvec{b})$ such that $||\myvec{a}||_2 = ||\myvec{b}||_2 = 1$, $\myvec{a}$ is orthogonal to $\mat{U}_1, \ldots, \mat{U}_{i-1}$ and similarly, $\myvec{b}$ is orthogonal to $\mat{V}_1, \ldots, \mat{V}_{i-1}$. 

In practice, CCA is carried out with two samples from $\rv{X}$ and $\rv{Z}$, and the correlation is calculated empirically.
The solution for CCA can be found by applying Singular Value Decomposition (SVD) on the empirical correlation matrix of the samples
of $\rv{X}$ and $\rv{Z}$. The singular values of these matrix correspond to the correlation values between the datapoints for each of the projected
directions. For more information, we refer the reader to \newcite{hardoon2004canonical}.


